Enlightening Flash Storage to Stream Writes by Objects

For a write request, today flash storage cannot distinguish the logical object it comes from. In such object-oblivious flash devices, concurrent writes from different objects are simply packed in their arrival order to flash memory blocks; hence objects with different lifetimes are multiplexed onto the same flash blocks. This multiplexing incurs write amplification, worsening the performance. Tackling the multiplexing problem, we propose a novel interface for flash storage, FlashAlloc. It is used to pass the logical address ranges of logical objects to the flash storage and thus enlighten the storage to stream writes by objects. The object-aware flash storage can de-multiplex writes from different objects with distinct deathtimes into per-object dedicated flash blocks. Given that popular data stores separate writes using objects (e.g., SSTables in RocksDB), we can achieve, unlike the existing solutions, transparent write streaming just by calling FlashAlloc upon object creation. Our experimental results using an open-source SSD prototype demonstrate that FlashAlloc can reduce write amplification factor (WAF) in RocksDB, F2FS, and MySQL by 1.5, 2.5, and 0.3, respectively and thus improve throughput by 2x, 1.8x, and 1.2x, respectively. In particular, FlashAlloc will mitigate the interference among multitenants. When RocksDB and MySQL were run together on the same SSD, FlashAlloc decreased WAF from 4.2 to 2.5 and doubled their throughputs.

==> 0.abstract.tex <==
\begin{abstract}
%Good English: 
% - The algorithms represent a simple way to augment existing database systems to MAKE their performance MORE ROBUST
% - IN THE PRESENCE of SKEWED JOINS. 
% - Analogy: e-mails are displayed in the order they arrived, not sorted/grouped/clustered by senders. 
% - Mails from different senders tend to interleave each other.
% - Blurring the Line Between OSes and Storage Devices Gregory R. Ganger December 2001 CMU-CS-01-166  Carnegie Mellon University ~\cite{Ganger01}

\comment{
Contact: Greg Ganger (ganger@ece.cmu.edu)~\cite{Ganger01}

This report makes a case for more expressive interfaces between operating systems (OSes) and storage devices. In today’s systems, the storage interface consists mainly of simple read and write commands; as a result, OSes operate with LITTLE UNDERSTANDING OF DEVICE-SPECIFIC CHARACTERISTICS and devices operate with LITTLE UNDERSTANDING OF SYSTEM PRIORITIES. MORE EXPRESSIVE INTERFACES, together with extended versions of today’s OS and firmware specializations, would allow the two to cooperate to achieve performance and functionality that neither can achieve alone.

In many cases, pages from the same file/object are very likely to have same death time. But, FTL does not have any knowledge about which page belongs to which file or object. By conveying simple, though limited, info (a set of logical LBAs belongs to the same XX), FlashAlloc can help flash storages to reduce  write amplification by grouping writes by object

With the hint from FlashAlloc, FTL can now manage page writes (in terms of physical space allocation and mapping management) in an ``object-associative'' way. <-- The existing FTLs are categorized into full- or set-associative in terms of LBA addresses.  ss   Note that fully-associative page mapping FTL as well as set-associative FTL are not object-associate, instead low-level page-associative!! 
}

\comment{
현재 SSD/FTL에서는, 쓰기 요청이 주어진 특정 논리 페이지가 어느 logical objects에 속하는 지에 관한 semantic information (엄밀하게는 구분할 수 있는 정보)가 없는 관계로, 호스트 쓰기 페이지들을 소속 논리객체에 따라 그룹핑 또는 클러스터링이 현실적으로 불가능하다. 즉, such semantic info 전달방법 부재. \falloc는 이러한 시맨틱 정보를 SSD/FTL로 직접 전달을 허용하고, SSD/FTl은 해당 시맨틱 정보를 바탕으로 주어지는 쓰기 요청에 대해 논리객체별로 서로 다른 물리 공간에 구분해서 클러스터링함으로써 (grouping/clustering writes by logical objects), ; deathtime에 따른 이상적인 placement --> lowering GC overhead/WAF --> we can achieve WAF close to 1, which is ideal.}

\begin{itemize}
%On-demand vs. Eager allocation of physical flash space.;; On-demand allocation and its problem: pages from different files with different lifetimes are multiplexed on to the same flash block. gc overhead
\item Given a write request with starting logical address and its data, every flash storage allocates physical flash space to store the given data on demand. With {\em on-demand allocation} of physical space, pages from multiple write streams each with different lifetime will be multiplexed onto the same flash blocks so that the writes will be amplified in the long run.;;  All current flash storages allocates physical space when write requests arrives. With this {\em on-demand} allocation, writes from different objects with different death times are mixed (or multiplexed) onto the same flash blocks for various reasons, consequently incurring high write amplifications even in many applications with flash-friendly write patterns.  

\item Flash storage are object-oblivious in handing writes because the semantic information about objects are not conveyed to it. thus, multiplex writes regardless of objects; consequently, writes are heavily amplified. (that is, writes from an object tend to scatter over different flash storage blocks while writes from different objects colocate in the same flash block.  As a consequence, as pages from objects with different death times are invalidated at different points of time, WAF will be high.)  FTL is oblivious to the belong-to relationship between LBA and segment/object/file.

\item In fact, applications as well as database engines and file systems implicitly or explicitly separate write streams. for instance, file/fallocate. In flash storage with no overwrite allowed and thus with indirection between logical and physical address. Unfortunately, there is no mechanism to propagate the potentially useful semantics about write streams to flash storage. (why: copy-on-write and another indirection b/w L and P.) Recall that, in contrast, harddisks with in-place-update allowed are, though implicitly, leveraging the information so as to physically cluster data pages by logical objects.;; In many cases Apps already distinguish write by logical objects. But, due to many complicated and interwoven factors such as on-demand allocation, concurrent writes, append, and splits, the semantics about writes by objects are, however, lost(?) along the kernel IO stacks to the flash storage and thus writes from diff objects are mixed with each other in the same flash blocks. As a result, because pages from different objects have different death times, seemingly flash-friendly write patterns also incur excessive internal write amplifications. 
%플래시메모리 저장장치는 호스트쓰기연산이 주어진 시점에, 해당 데이터를 저장할 물리적 공간을 할당하고 쓰기를 진행한다. 이러한 온디맨드 할당 (on-demand allocation) 정책은, 동일 플래시블록에 서로 다른 화일에 속하는 페이지들이 위치하게 하고, 생명주기(lifetime)가 다른 화일들이 다른 시점에 삭제되기 때문에 장기적으로 플래시메모리의 쓰기증폭을 심화시킨다. 

\item Though limited to the logical address ranges, {\bf the semantic of objects provided by applications and conveyed to flash storage} is critical to making flash storages reduce write amplification effectively and significantly across many data-intensive applications.

\item logical segment whose pages will be dead together 정보를 SSD에 전달해서, segregate those pages into dedicated physical block NAND and erased together, thereby reducing write amplification, increasing write performance and enhancing the life time of flash storage. 

\item For FTL to be able to distinguish and thus group writes by logical objects, we propose a novel interface for flash storage, so called \falloc.

%\falloc - simple but novel and powerful abstraction to address many SSD- and SW-stack-related inefficiency.
\item To rectify the problem(loss?), we propose a novel interface \falloc for flash storage, which informs flash storages that the given set of pages belongs to the same objects. Upon receiving \falloc, flash storage preempts a dedicated flash block(s) for the given page set in advance and later store every writes from the set in the corresponding block.; To remedy this XX, we propose a new interface for flash storage, FlashAlloc, which can convey the semantic information about object to the flash storage. With the help of FlashAlloc, flash storage can now understand which LBA belongs to which object so that it will group/cluster writes by objects, thus lowering WAF.;;
As a solution to remedy this problem, this paper propose a new interface for flash storages, called {\em flash-allocate (\falloc in short)}, which is used to ask to allocate physical flash storage in advance for logical address ranges. Since the physical space is already allocated in advance, a following write for the \falloc-ed logical address will be written to the physical space so that pages from multiple write streams with different lifetimes are de-multiplexed onto its dedicated flash blocks. With the help of \falloc, the write amplification can be minimized.  

%논리주소범위에 대해 동일 플래시메모리 블록(들)에 선 할당 (eager allocation)하는 플래시메모리 저장장치 인터페이스 \falloc (flash allocate 줄임말) 기법에 관한 것이다. 응용으로부터 논리주소범위에 대해 \falloc 요청이 주어지면, 플래시메모리 저장장치는 해당 주소범위에 물리공간을 미리 할당하고, 이후 해당 논리주소범위에 속하는 페이지의 쓰기요청 발생시 선할당된 물리공간에 쓰게 된다. 

With \falloc properly used, writes from different objects are streamed to its corresponding flash block so that ....., thus reducing write amplification and prolonging the lifespan of the flash storage. 
%falloc 통해서 해당 논리범위에 속하는 페이지들이 동일 물리공간에 클러스터링되고 다른 페이지들과는 분리저장되므로 장기적으로 저장장치의 쓰기증폭을 줄여 쓰기 성능 및 수명을 향상시킨다. 

%VALUE OF \FALLOC: 1. Flash에서 LBA ranges를 통해 동일 object에 대한 hint를 현재 eco에서 그대로 전달하게 해서, 2. "sync or async"하게 해당 range가 동일 physical block(s)에 클러스터링되게 함으로써, 3. WAF 최소화하는 메커니즘. 
\item The main goal of \falloc is to minimize WAF by preventing {\em write multiplexing} and thus maximize the sustained performance of flash storage. \falloc: Preempting physical space to prevent write multiplexing in flash storages; Eager allocation of physical flash block or space to logical address ranges thus de-multiplexing different write streams with different death time  so that each file data is isolated or clustered into different  block when deleted or overwritten an entire flash block is erased. 

\end{itemize}

\end{abstract}


==> 1.intro2.tex <==
\section{Introduction}

% SW system object별 write 구분; object별 fallocate 통해 연속된 논리 주소 공간 확보를 통해 객체별 데이터의 클러스터링, 
% HDD 경우 in-place-update로 인해, 논리 주소 공간과 물리 주소 공간 사이 1:1 대응이 됨. 따라서, object별 write가 split되고, interleave되어도, 원래 implicitly allocated physical space에 할당  
% HDD: overwrite -> aligned: physical space IMPLICITLY/STATICALLY/In-Advance alloced upon falloc (L2P 1:1 mapping) 

% object 사용 data 관리; logical space per object; same death time upon object deletion. 
Most software systems, including LSM (Log-Structured-Merge) tree-based KV (Key-Value) stores, relational DBMSs, and file systems manage data using logical objects: to name a few, SSTables in RocksDB, DWB (double write buffer) in MySQL, and segments in F2FS. And, upon each object creation, its logical space is secured in advance before writes are made to the object. For instance, RocksDB calls {\tt fallocate()} right after creating an SSTable file so as to secure the logical address space for the file. The logical address range allocated from the call belongs to the file object. For this reason, from an LBA address, the host-side data stores can identify its belonging object. In addition, when an object is deleted, all its data will be invalidated together at once; thus the data set belonging to an object is said to have the same deathtime. Meanwhile, different objects are, though created and populated simultaneously, usually destructed at different points in time; they have different deathtimes. 
%For example, SSTable files in RocksDB will be compacted and deleted at different points of time. \comment{Segments in F2FS will be also cleansed at different points of time.} 
In summary, host software stacks manage data by objects; each object is the unit of logical space allocation and, in many cases, all its pages will have the same deathtime.

% on-demand physical space allocation --> thus, {\bf multiplexed}. 
%On-demand vs. Eager allocation of physical flash space.;; On-demand allocation and its problem: pages from different files with different lifetimes are multiplexed on to the same flash block. gc overhead
%- CONCURRENT WRs will be multiplexed ON SSD:  pages with diff. death time in same flash blocks --> copyback at GC -> high WAF
%- 특히, independent multiple write threads / multi-tenant --> multiplexing/WAF inevitable!

\begin{figure}[h]
\centering
\includegraphics[clip,width=0.43\textwidth]{figure/salloc-archi.eps}
\caption{Object Placement: Multiplexing vs. Clustering}
\label{fig:sallocate-archi}
\end{figure}

Though host software stacks can distinguish objects by their logical address ranges, the host-side semantic about objects' logical address ranges cannot cross the storage interface wall simply because no interface exists to pass it to the storage. As a result, today's flash storage has no knowledge about the belongs-to relationship between LBA address and object. Therefore,  when concurrent writes from different objects interleave, the conventional {\em object-oblivious} flash storage cannot distinguish each write's object so that it has no choice but to simply append new data in their arrival order into flash blocks. As a consequence, writes from different objects colocate in the same flash blocks. That is, each flash block will be multiplexed by data from multiple objects with different deathtimes, as illustrated in Figure~\ref{fig:sallocate-archi}. We call this situation as {\em multiplexing}. 
%\reminder{Therefore,  when concurrent writes from different objects interleave, the conventional {\em object-oblivious} flash storage cannot distinguish each write's object but instead will simply pack new data in their arrival orders into flash blocks. --> (1) cannot distinguish each write's object but instead 는 object-oblivious와 같은 말이므로 삭제해도 될 것 같습니다. (2) 다문장에 동일 블록에 섞인다는 말이 있으므로 pack ~ info flash blocks 보다 2장의 표현처럼 append new data in their arrival orders 가 의미 전달에 더 좋을 것 같습니다}

%flash storage will allocate physical space on demand for the incoming write requests originating from different objects in their arrival orders onto striped multiple channels. With such {\bf {\em on-demand allocation}} of physical space, writes from an object tend to scatter over different flash storage blocks while writes from different objects colocate in the same flash block. 

\subsection{Multiplexing}
The multiplexing is the main culprit of physical write amplification in flash storage, worsening the performance and lifespan of flash storage. Since logical objects have different deathtimes each other in most cases (\eg, four SSTables in Figure 1 will be deleted at different points of time), pages in a multiplexed flash block will be incrementally invalidated at different points of time. When the block is chosen as a victim for garbage collection, the remaining valid pages have to be relocated to another block, amplifying physical writes inside flash storage. In particular, contrary to the common belief, the multiplexing will make even RocksDB and F2FS taking sequential write patterns suffer from severe device-level write amplification~\cite{DONOTSTACK,AMF,VLDB21FlashSSDs}. 
According to our experiments using commercial SSDs, write amplification factor (WAF in short) becomes even greater than 
eight (Figure~\ref{fig:f2fs-on-micron}). 
%culprit for high waf even for flash-friendly softwares. 
In this sense, the so called {\em flash-friendly} sequential writes are {\em not less harmful} than random ones in the conventional flash storage~\cite{SFS}.
\comment{ In particular, since {\bf random writes are considered harmful} in Flash~\cite{SFS}, numerous database/file systems such as RocksDB and F2FS taking flash-friendly sequential writes have been proposed and become popular. Contrary to the belief/expec. that seq WR is good for flash, however, even such softwares also suffer from high WAF~\cite{AMF, VLDB21FlashSSDs, ++}. 많은경우 sequential write 선호 systems서도, OLTP random write comparable WAF 관찰됨: >= 2, in some cases, up to 6!.  the unexpected multiplexing, despite of logically sequential writes against each object, is attributable to several reasons such as concurrent writes, split, append-only writes, striped write, ever-increasing block and channel size; 각 objects with different lifetimes and sequential write patterns are also multiplexed, thus experiencing excessive write amplification.
} 
In addition, the multiplexing can exacerbate the performance interference in multi-tenant environment~\cite{SeattleReport}. When multiple applications, each with its set of objects, are run together on a flash device, more objects with more deviating deathtimes will be multiplexed onto the same flash blocks, worsening write amplification.  

\comment{
To sum up, since no interface exists to offload the host semantic about objects' logical address range to the storage, the valuable semantic is discarded and the object-oblivious flash device can not stream writes by objects, incurring multiplexing and write amplification. 
}

\subsection{Missing Interface}~\label{sec:pd}

Consider why existing flash devices should be object-oblivious in handling writes and thus incur the multiplexing problem. The main reason is that, from the logical address in a write request, flash storage can not distinguish the logical object the address belongs to.
This is in turn because the conventional block interfaces do not provide any mechanism to pass the relationship between objects and their logical address ranges to the storage. That is, while the host software stacks are aware of the relationship, the valuable semantic cannot cross the storage interface wall but is simply discarded. In this sense, we say that a crucial semantic interface is missing which can make flash storage object-aware. Note that the absence of such useful interface is due to the legacy that the existing storage interfaces have been developed assuming harddisk. In the case of harddisk where overwrites are allowed, logical space allocation via the {\tt fallocate()} call at the file system layer implicitly indicates physical space allocation at the storage.
Thus, writes from the host will go to their corresponding physical location simply according to their {\tt start\_lba}s: harddisk is object-aware in handling writes without any hint from the host. For this reason, no storage interface was in need, which can pass the host semantic about object's address range to the storage. This unwritten contract fails on SSDs where overwrites are not allowed.

% SSD: unlike HDD where phys. space is allocated implicitly upon fallcate(). 
% no overwrite/copy-on-write --> physical space ON-DEMAND allocated upon WR at PM-FTL
% Object-Oblivious SSD: LogicalAddress - Object relationship info missing!! --> Given logical writes, no semantics about LBAs and objects --> Multiplexing; Thus, can't group pages into diff. blks by object;; instead, on-demand physical space alloc.(+cite)!     
% (on-demand allocation) 정책은, 생명주기가 다른 화일 데이터들을 동일 플래시블록에  위치시키고, as those pages are incrementally invalidated over time, 장기적으로 플래시메모리의 쓰기증폭을 심화시킨다. 
%\falloc - simple but novel and powerful abstraction to address many SSD- and SW-stack-related inefficiency.
%{\bf For objects such as fallocate, DWB, F2FS segments, 해당 logical address range가 same object에 속하는 semantic을 convey}. 

%host semantic -> interface -> object-aware -> (also) dedicate blocks -> stream writes by blocks -> preventing multiplexing;
%With the help of \falloc, flash devices becomes {\bf object-aware} in the sense that they, at least, an LBA address가 주어졌을 때 어떤 FA instance에  속하는지 구분가능 and thus eventually able to group writes by object to its dedicated flash blocks (\ie, stream writes by objects), de-multiplexing writes: thus preventing write amplification upon GC due to the multiplexing and thus drastically reducing write amplification and maximizing its lifespan as well as sustained performance. 
%((semantic info. loss -> \falloc will fill/preserve/propagate the {\em semantic gap}  bw app/fs/dbms and flash storage.)) 

\subsection{FlashAllocate}
Addressing the multiplexing problem, we propose a novel interface, {\em FlashAllocate} (\falloc in short), which is used to pass the host semantic about object's logical address range to the flash storage and thus to enlighten the storage to be {\em object-aware} in handling writes. 
%the belong-to relationship semantic between LBAs and object to flash Storage; To cluster writes by object and prevent multiplexing, 
To be concrete, after creating an object, a data store calls \falloc with the object's local address range as a parameter to inform the flash device that the address range belongs to the same object. Then, upon receiving \falloc, the flash device creates a corresponding FlashAlloc (FA in short) instance, which keeps the given range information and thus is now aware of the address range of the object. At the same time, the flash device will secure physical flash block(s) where to place writes from the object and dedicate those blocks to the FA instance. Hereafter, the logical address range of an \falloc call has its corresponding physical space. For each write request, \comment{(from an \falloc-ed range)} flash storage probes its matching FA instance, if it exists, using the starting LBA address of the request and then stream the write to the dedicated blocks for the FA instance. %now leverage the semantic in clustering writes coming from the range into the same flash block(s). 
%... flash storage secures/pre-allocates(not on-demand)/preempt/dedicates clean physical flash blocks to the given logical address range in advance (either eager or lazy/delayed/on-demand allocation) before new writes to the logical pages are made. 

%Enlightened by \falloc, the flash device can stream writes by objects. That is,  the flash storage can de-multiplex writes from different objects with distinct deathtimes into per-object dedicated flash blocks, thus preventing the write multiplexing of different objects into the same flash blocks and lowering WAF.

Once logical objects are \falloc-ed, their writes will be, as illustrated in the right bottom of Figure~\ref{fig:sallocate-archi}, de-multiplexed into per-object dedicated flash blocks.\comment{Also, different objects will not share the same flash block but each object's data is isolated into distinct block(s)} In this regard, we say that flash storage, enlightened by \falloc, can stream writes by objects. The write streaming by objects is a natural way to achieve {\em grouping data by deathtime}~\cite{UnwrittenContract} because logical objects have different deathtimes while all pages of an object become dead together at once upon the object destruction. 
Thus, the ultimate benefit of streaming writes by objects is to avoid GC-induced write amplification. For instance, as each SSTable file is deleted in Figure~\ref{fig:sallocate-archi}, all its pages are invalidated, and thus, its dedicated block can be erased in its entirety, not causing any page relocation.
In summary, \falloc provides an alternative in {\em controlling the physical placement of writes} inside flash devices: it enables to de-multiplex logical objects into the different flash block(s) just resorting to the already-existing host-side object semantic and thus without introducing other intermediate concepts such as stream-id or zone-id~\cite{MultiStreamSSD,ZNS}. 

%its all pages remain intact and valid from their birth to death so that their flash blocks will not be selected as victims for GC and will be simply erased in their entirety later upon the object deletion and returned as free, thus incurring no physical write amplification.;; flash blocks will contain pages which will be dead altogether at once upon deletion of the object they belong to. upon object deletion, its dedicated flash blocks are invalidated at once and simply erased/returned as free blocks; in this way, 

Whilst effectively de-multiplexing objects with sequential write-once pattern, \comment{ into different flash blocks,} \falloc is not a panacea for the write amplification problem. In particular, \falloc is not intended to be used for objects with random overwrites (\eg, relational database's tablespace under OLTP workload). For non-\falloc-ed objects, their data will be stored in non-FA instance and managed by the conventional FTL. In this way, flash storage supporting \falloc can support two types of objects, objects with sequential writes and objects with random overwrite, concurrently. In this respect, \falloc is in stark contrast with the Zoned Name Space (ZNS) interface, which forces applications to follow the strict sequential write rule~\cite{ZNS}. 
% de-multiplexing different write streams with different death time so that each file data is isolated or clustered into different block, when deleted or overwritten an entire flash block is erased. 

%VALUE OF \FALLOC: 1. Flash에서 LBA ranges를 통해 동일 object에 대한 hint를 현재 eco에서 그대로 전달하게 해서, 2. "sync or async"하게 해당 range가 동일 physical block(s)에 클러스터링되게 함으로써, 3. WAF 최소화하는 메커니즘. 

\falloc is similar to the {\tt trim} command~\cite{trim}: both aim at reducing write amplification by hinting flash device about host semantics (\ie, logical address range allocated upon object creation and staled upon object deletion, respectively). Interestingly, when used together, they are synergetic to reduce write amplification further. 
%at no or minimal change in the existing software stacks, (In a sense, they have duality.) 
%\reminder{Trim and \falloc on HDD vs. Flash: 언급필요?}
% Note that \falloc-like interface was not explicitly required with harddisk where LBA ranges are allocated to the same physical space because overwrites are allowed. In contrast, with flash storage with overwrite not allowed, the \falloc interface is further required to explicitly convey the information that an LBA range belong to the same object. 
% 기존기법 핵심차이: stream 구분위해 ms-ssd stream-id 필요; 반면, falloc은 사용자 부담없이 자연스러운 streaming!
Meanwhile, the \falloc interface might not be such novel considering there already exists a write streaming interface, MS-SSD~\cite{MultiStreamSSD}. Unlike MS-SSD resorting to the stream-id concept, \comment{intermediate concept of stream-id,} we can stream writes \comment{at the grain of objects} simply by calling \falloc after object creation. Thus, developers are free from the burdens of determining the proper number of streams, grouping objects into limited streams, and assigning stream-id to every write call. Also, \falloc will not incur the stream-id conflict among multi-tenants. In this sense, \falloc is a simpler and more advanced abstraction than MS-SSD, enabling transparent write streaming.

\reminder{
(R3:D2) "FlashAlloc will not incur the stream-id conflict among multi-tenants" does not seem an important advantage, as it could be easily avoided by either having a unique prefix for each application or using psudo-random stream IDs.";
(R1:D2) "Can't one use NVMe namespaces to separate address spaces for different tenants already"; 
namespace로 분리하는 것은 logical isolation만 달성할 뿐이며, physical isolation (e.g., IOD device)은 달성할 수 없음. 
FlashAlloc이 MS-SSD에 비해가지는 장점 상세히 명시 필요; host application이 stream id assign을 잘 했더라도 
GC 또는 wear-leveling 과정에서 stream id가 섞일 가능성이 있음. stream ID 갯수는 제한된다는 점 강조 필요!!! 
기존기법 핵심차이: stream 구분위해 ms-ssd stream-id 필요; 반면, falloc은 사용자 부담없이 자연스러운 streaming!
}


\comment{
\begin{itemize}
\item {\bf bf Concurrent Write Threads, Write Split, fallocate후 append } 또한, 동시 write, write split, append 되기 때문에, 위 ON-DEMAND allocation과 결합되어서, 서로 다른 file page들이 한 flash block에 섞이게 되고, thus pages belonging to a file or a logical object are multiplexed onto different flash blocks (Figure~\ref{fig:sallocate-archi} (a)). 
\item {\bf On-demand physical space allocation in SSD} 또한, flash storage는 out-of-place write 특성으로 인해, 실제 write 요청이 왔을 때, ON-DEMAND로 physical address space가 allocation된다.
\item {\bf SSD RAID striping} split 2MB --> into 8 * 256KB  
\item FS Fragmentation:  1) LBA fragmentation; with buffered writes, when a file consists of N fragmented LBAs, then N writes will be made scattered? 2) Unless a file is LBA-fragmented, a large sequential write made at page cache layer can be split into multiple write calls, along the IO stack, thus causing N write commands to the storage.
\item unit mismatch between fallocate and write, and write 시점이 다름.  
\end{itemize}
}

\subsection{Contributions}
The main contributions of this paper are summarized below.
\textcircled{\small 1} We make an observation that data stores with flash-friendly write patterns, contrary to the common belief, experience severe write amplification on conventional SSDs and investigate the write multiplexing as the main culprit for the problem. We also show that the write multiplexing makes multi-tenants interfere with each other. 
\textcircled{\small 2} We motivate that existing flash devices are object-oblivious simply because the host semantic about the object's logical address range cannot cross the storage interface wall. 
\textcircled{\small 3} Based on this motivation, we propose a new interface, \falloc, which allows to offload the host semantic about object's logical address range to the storage and thus to enlighten flash device to be able to stream writes by objects, reducing device-level write amplification. We also suggest an extended design of page-mapping FTL to support.
\textcircled{\small 4} The abstraction used in \falloc is so simple and intuitive that existing software stacks can realize the write streaming by objects \comment{nearly in a transparent way} with minimal or even no change in its codebase.
\textcircled{\small 5} We have prototyped \falloc using the Cosmos open-source SSD. Our experimental results show that \falloc can reduce WAFs in RocksDB, F2FS, and MySQL by 1.5, 2.5, and 0.3, respectively, and accordingly improve throughput by 2x, 1.8x, and 1.2x, respectively. In particular, when RocksDB and MySQL are run together, \falloc can reduce WAF from 4.2 to 2.5, and doubled their throughputs. \comment{improve RocksDB's OPS by 2x and MySQL's TPS by 2x, respectively.}

%The main {\bf contributions} of this paper can be summarized as follows.
% - 중요현상파악/원인분석/problem define!
% - novel solution: covering design/impl.
%  - comprehensive exp -> 유용성 확인!
%  - log-on-log 등 주요문제 simple, fundamental solution.

%% DO NOT REMOVE %% 
\comment{
\begin{itemize}
\item We make an observation that data stores with flash-friendly write patterns, contrary to the common belief, experience severe write amplification on conventional SSDs and investigate the write multiplexing as the main culprit for the problem. We also show that the write multiplexing makes multi-tenants interfere with each other. 

\item We motivate that existing flash devices are object-oblivious \comment{in handling writes} simply because the host semantic about the object's logical address range cannot cross the storage interface wall. 
%\item We motivate that conventional flash devices are object-oblivious in handling writes simply because no interface exists to offload the host semantic about objects' logical address range to the underlying storage. 

\item Based on this motivation, we propose a new interface, \falloc, which allows to offload the host semantic about object's logical address range to the storage and thus to enlighten flash device to be able to stream writes by objects, reducing device-level write amplification. We also suggest an extended design of page-mapping FTL to support \falloc. 

\item The abstraction used in \falloc is so simple and intuitive that existing software stacks can realize the write streaming by objects \comment{nearly in a transparent way} with minimal or even no change in its codebase.

%\item {\bf Object-oblivious flash 문제 root cause 규명}: logical vs. physical 관계 전달 interface 부재 (hdd서는 불필요 but flash서는 inevitable interface)에 따른 {\bf multiplexing}임 규명.

%As a result, in case of flash storage, write stream of a file is split (due to various reasons) and multiplexed into different flash block so that segments from different files colocated in the same flash block.

%fallocate call을 하는 rocksDB는 전혀 수정 필요없음. 2MB alignement하면 더 나은 결과! DWB의 경우, MySQL/InnoDB에 \falloc call 관련 (10줄 이내) 추가! side-benefit 간단 언급(?)
\comment{in modern data intensive applications (even known as flash-friendly database storage engine/file system). }

%\item We enumerate several {\bf design issues}, discuss their alternatives and explain our choices. Also, a few optimizations. % such as sync vs. async processing; row/column-wise allocation;  any other optimization?

\item  We have prototyped \falloc using the Cosmos open-source SSD. Our experimental results show that \falloc can reduce WAFs in RocksDB, F2FS, and MySQL by 1.5, 2.5, and 0.3, respectively, and accordingly improve throughput by 2x, 1.8x, and 1.2x, respectively. In particular, when RocksDB and MySQL are run together, \falloc can reduce WAF from 4.2 to 2.5, and doubled their throughputs. \comment{improve RocksDB's OPS by 2x and MySQL's TPS by 2x, respectively.}
%\item  Finally, we have {\bf prototyped \falloc} on a real commercial-grade openSSD and carried out a {\bf comprehensive set of experiments} running diverse/popular write-intensive  RocksDB, F2FS, MySQL, and multi-tenant scenarios on SSD with/without \falloc. Our experimental results using various database applications confirm that \falloc can, compared to ORG, reduce the write amplification in XXX by one fourth, thereby tripling IO performance and transaction throughput and improving tail-latency. In the case of F2FS and MySQL,.. In particular, even when only RocksDB was \falloc-ed while other tenants are not, its performance was doubled while that of MySQL was trippled(?). In this sense, we would like to say that \falloc is not only beneficial to the caller itself but also in many cases altruistic to other neighboring tenants. 
\comment{Our experimental results across a comprehensive set of representative workloads confirm that \falloc can, compared to the existing on-demand allocation, significantly reduce write amplification, thus considerably improve throughput and latency. In particular,  when applied to multi-tenant workloads of Rocksdb and MySQL, \falloc can reduce total WAF from 5 to 1.5, and improve OPSs by 3x and 2x for RocksDB and MySQL, respectively. ...} 
\comment{For this, we modified F2FS and MySQL/InnoDB minimally to call the \falloc while RocksDB at no change.} 
\comment{Using various representative use-case applications as well as multi-tenant scenarios. Our result are very promising., including 1) explicit fallocate call, 2) segment write at LFS file system, 3) DWB@InnoDB/RBJ/WAL@SQLite etc., 4) synthetic FileBench/varmail ( large sequential write(s) (even w/o explicit fallocate call) @ page cache; 5) multi-tenant (RocksDB / MySQL). 성능개선정도 언급!
fallocate()통해 \falloc을 호출하면, 해당 응용 자체 성능개선 외에, 동일 SSD를 공유하나 fallocate을 호출하지 않는 다른 응용들의 데이터들과 다른 플래시블록에 분리 저장되어서 SSD 쓰기증폭이 줄어들어 궁극적으로 모든 응용의 성능 개선에 도움이 될 수 있다. 응용 with \falloc would be altruistic to other applications. 
}
\end{itemize}
}



%In that \falloc passes the host semantic that a logical address range belongs to the same object to the flash device so as to reduce write amplification, it is similar to the {\tt TRIM} interface~\cite{trim} which notifies the stale data at the file system to the flash device for the same purpose. 
%%% DO NOT REMOVE %%%%%
\comment{
\falloc is similar to the {\tt trim} command~\cite{trim}: both aim at reducing write amplification by hinting flash device about host semantics (\ie, logical address range allocated upon object creation and staled upon object deletion, respectively). Interestingly, when used together, they are synergetic to reduce write amplification further. 
%at no or minimal change in the existing software stacks, (In a sense, they have duality.) 
%\reminder{Trim and \falloc on HDD vs. Flash: 언급필요?}
% Note that \falloc-like interface was not explicitly required with harddisk where LBA ranges are allocated to the same physical space because overwrites are allowed. In contrast, with flash storage with overwrite not allowed, the \falloc interface is further required to explicitly convey the information that an LBA range belong to the same object. 
% 기존기법 핵심차이: stream 구분위해 ms-ssd stream-id 필요; 반면, falloc은 사용자 부담없이 자연스러운 streaming!
Meanwhile, the \falloc interface might not be such novel considering there already exists a write streaming interface, MS-SSD~\cite{MultiStreamSSD}. Unlike MS-SSD resorting to the stream-id concept, \comment{intermediate concept of stream-id,} we can stream writes \comment{at the grain of objects} simply by calling \falloc after object creation. Thus, developers are free from the burdens of determining the proper number of streams, grouping objects into limited streams, and assigning stream-id to every write call. Also, \falloc will not incur the stream-id conflict among multi-tenants. In this sense, \falloc is a simpler and more advanced abstraction than MS-SSD, enabling transparent write streaming.

\reminder{
(R3:D2) "FlashAlloc will not incur the stream-id conflict among multi-tenants" does not seem an important advantage, as it could be easily avoided by either having a unique prefix for each application or using psudo-random stream IDs.";
(R1:D2) "Can't one use NVMe namespaces to separate address spaces for different tenants already"; 
namespace로 분리하는 것은 logical isolation만 달성할 뿐이며, physical isolation (e.g., IOD device)은 달성할 수 없음. 
FlashAlloc이 MS-SSD에 비해가지는 장점 상세히 명시 필요; host application이 stream id assign을 잘 했더라도 
GC 또는 wear-leveling 과정에서 stream id가 섞일 가능성이 있음. stream ID 갯수는 제한된다는 점 강조 필요!!! 
}
}

%by exploiting the existing but valuable logical object 정보, \falloc enables the transparent and correct write streaming while the latter requires the intermediate abstraction of stream-id for write streaming \reminder{thus, program modification and complex task for identifications of write streams}. stream vs. object (fine-grained); more practical?) Therefore, allows applications to transparently realize the full potential of write streams at no program modification or further optimization overhead. 
%Since file system kernels or database storage engines just need to invokes the \falloc command against SSDs upon {\tt fallocate} or other use cases (\eg, DWB, segment alloc in F2FS), the existing software echo, write streams. --> a practical/effective solution to the multiplexing problem. 
%In addition, \falloc could be fundamental solutions to several flash-related problems, including log-on-log problem~\cite{DONOTSTACK}, proper address for by-death-time without segmented FTL~\cite{UnwrittenContract}, and anything else?. 

\comment{
\module{vs. Related Work - better abstraction and more practical} unlike MS-SSD, \falloc is 1) no limits in stream \#, 2) no mapping overhead b/w object-stream \#, 3) no (or minimal) s/w modification. \comment{In addition, though pages from one file are streamed into the same stream, they can be still spread over multiple flash blocks, thus causing waf!;} stream abstraction instead of object.(though object can be used as stream) - not-intuitive (stream - object mapping by application developer) + \# of streams << object; Unlike the existing stream separation scheme such as MS-SSD, \falloc will store different streams into different flash blocks in a very natural way, thus requiring no additional user intervention in assigning stream ids to each write stream and ++. (in theory unlimited number of streams, thus no limitation x) The \falloc interface can be easily and seamlessly integrated into the existing software eco systems. That is, as long as the existing applications call for {\tt fallocate} file system call with logical address, (and the system call internally invokes the corresponding \falloc command, the benefits of \falloc can be exploited. In addition, compared to {\bf host-managed SSD approaches} such as ZNS, OC-SSD, and AMF~\cite{AMF,OCSSD,ZNS}, no host/application overhead, no sw echo change (sequential write)  

{\bf Related work:} Compared to MS-SSD, \falloc provides {\bf better abstraction} for streaming and is {\bf more practical} solution particularly for multi-tenant environment with dynamic and unpredictable streaming requirement. In addition, compared to host-managed SSD solutions such as OC-SSD and ZNS which require radical and holistic changes across the stacks, \falloc is evolutionary and compliant to the existing stack. 
- unlike MS-SSD: 1) no limits in stream \#, 2) no mapping overhead b/w object-stream \#, 3) no (or minimal) s/w modification -- in addition, though pages from one file are streamed into the same stream, they can be still spread over multiple flash blocks, thus causing waf!; - unlike application/host managed solutions such as ZNS, OC-SSD, and AMF; no host/application overhead, no sw echo change (sequential write)  
}
%%% Side contribution: 2장 merge 후 간단 언급 --- DO NOT DELETE 
\comment{아래 내용 들
We make an important observation about the multiplexing of sequential write streams in many applications. and show that the effect of multiplexing on write amplification, performance degradation/performance variability and shortened lifetime is quite serious. Even in a single application such as RocksDB with of multiple concurrent write threads, Sequential writes at the application layers are not sequential at the block trace or FTL layers but instead splited and thus mixed with other stream chunk. In DWB; in log structured file systems, In the case of multi-tenants, the multiplexing is more outstanding. (HotStorage20 submit참고@Fallocate폴더@논문서버) ++++++ 그리고, investigate why logical objects are multiplexed into different flash blocks. 

\begin{itemize}
\item {\bf Concurrent Sequential Writes are Multiplexed:} We made an {\bf important observation} that logical objects with sequential write patterns are multiplexed to different flash blocks and thus they also suffer from high WAF in many softwares; Also, we investigate/explain why sequential write streams are multiplexed. 
{\bf Multiplexing~\cite{DONOTSTACK}:} ``Mixed workload from logs and other traffic destroys sequentiality – Each log writes sequentially, but the device gets mixed workload, most likely to be random – Underlying flash-based SSD also writes its own metadata.Multiple logs on a shared device results in random traffic seen by underlying device.'' (see also the slides at https://www.usenix.org/sites/default/files/conference/protected-files/inflow14\_slides\_yang.pdf)
\item {\bf Multiplexing effect:} Later, they are invalidated upon deletion or overwrite. As a result, contrary to the expectation, many applications suffer from high write amplification (NOTE: This observation is not widely known. Simply they assume that sequential writes are good for flash storage.) +  {\bf Log-on-log~\cite{DONOTSTACK} 언급} {\bf Why Multiplexex:} 보기에 sequential write (즉, 같은 object에 대해 긴 write가 주어졌을때, 이들이 같은 flash blocks에 clustering 되지 않고 다른 block들에 흩어짐, for various reasons such as on-demand allocation, file system fragmentation, SSD architecture, and write split~\reminder{2장 관련 정리 후, 여기서는 simply enumerate할 것}. For this reason, 실제 seq- wr 요청하는 다양한 application들에서 서로 다른 deathtime/lifetime을 가지는 file or objects들의 data pages들이, not clustered but multiplexed into flash blocks;
\end{itemize}
}

\comment{\module{Misc.}  
1.Terminology: page and its belonging object; object and its pages
2. Object(File, Table) vs. segment(or chunk/extent, unit of logical space allocation at FS or database)  vs. pages, blocks VS. host에서 logically fallocate 단위. 같은 file도 two or more fallocate 가능. finer granularity!! eventually, pages from different objects will not mix with each other in the same flash block.;
3. An object may consist of one or more segments, and a segment has a set of logical pages (mostly contiguous, but not always) .. {\bf For the simplicity of discussion, we regard every object calls one {\tt fallocate} at its creation time, which is true in many cases such as RocksDB SSTable, F2FS segment, and DWB. But, \falloc does not exclude the case where an object call multiple \falloc. Recall that each segment is streamed into diff blocks, we still guarantee that {\bf group by objects}}  
4. falloc vs. fallocate(): 다른 layers/roles, 단, fallocate -> \falloc 호출
5. that logical segment whose pages will be dead together at once to SSD, segregating those pages into dedicated physical block NAND. 6. (regardless whether pages from a file are written scatteredly in time (by application) or one large sequential write is split into multiple segments by kernel (fragmentation or IO stack), a write segment from a file object is eventually merged into the same flash block.} 
